Order Fairness Evaluation of DAG-based ledgers

Order fairness in distributed ledgers refers to properties that relate the order in which transactions are sent or received to the order in which they are eventually finalized, i.e., totally ordered. The study of such properties is relatively new and has been especially stimulated by the rise of Maximal Extractable Value (MEV) attacks in blockchain environments. Indeed, in many classical blockchain protocols, leaders are responsible for selecting the transactions to be included in blocks, which creates a clear vulnerability and opportunity for transaction order manipulation. Unlike blockchains, DAG-based ledgers allow participants in the network to independently propose blocks, which are then arranged as vertices of a directed acyclic graph. Interestingly, leaders in DAG-based ledgers are elected only after the fact, once transactions are already part of the graph, to determine their total order. In other words, transactions are not chosen by single leaders; instead, they are collectively validated by the nodes, and leaders are only elected to establish an ordering. This approach intuitively reduces the risk of transaction manipulation and enhances fairness. In this paper, we aim to quantify the capability of DAG-based ledgers to achieve order fairness. To this end, we define new variants of order fairness adapted to DAG-based ledgers and evaluate the impact of an adversary capable of compromising a limited number of nodes (below the one-third threshold) to reorder transactions. We analyze how often our order fairness properties are violated under different network conditions and parameterizations of the DAG algorithm, depending on the adversary's power. Our study shows that DAG-based ledgers are still vulnerable to reordering attacks, as an adversary can coordinate a minority of Byzantine nodes to manipulate the DAG's structure.

==> 3_4_old.tex <==

\iffalse 
\begin{figure}[h]
    \centering

\begin{subfigure}{.15\textwidth}
    \centering
    \scalebox{.8}{\input{figures/deterministic/do_example_simpl}}
    \caption{DAG}
    \label{fig:do_example_simpl_dag}
\end{subfigure}
%
\begin{subfigure}{.3\textwidth}
    \centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{} & \multicolumn{4}{c|}{earliest vote by} \\
\cline{2-5} 
     & $n_0$ & $n_1$ & $n_2$ & $n_3$ \\
     \hline 
$v_4^0$ & $4$ & $6$ & $\infty$ & $\infty$ \\
\hline 
$v_5^0$ & $5$ & $6$ & $\infty$ & $\infty$ \\
\hline 
$v_4^1$ & $5$ & $4$ & $\infty$ & $\infty$ \\
\hline 
$v_5^1$ & $\infty$ & $5$ & $\infty$ & $\infty$ \\
\hline 
$v_6^1$ & $\infty$ & $6$ & $\infty$ & $\infty$ \\
\hline 
$v_4^2$ & $\infty$ & $5$ & $\infty$ & $\infty$ \\
\hline 
$v_4^3$ & $\infty$ & $6$ & $\infty$ & $\infty$ \\
\hline 
\end{tabular}
    \caption{Vote table}
    \label{fig:do_example_simpl_votes}
\end{subfigure}
    
    
    \caption{Simplified example with $2$ strong edges per vertex}
    \label{fig:do_example_simpl}
\end{figure}
\fi 

==> figures/deterministic/do_example.tex <==
\begin{tikzpicture}
\node[draw] at (0,0)                  (v04) {$v^0_{4}$};
\node[draw,        below=.3cm of v04] (v14) {$v^1_{4}$};
\node[draw,        below=.3cm of v14] (v24) {$v^2_{4}$};
\node[draw,        below=.3cm of v24] (v34) {$v^3_{4}$};
\node[draw,        below=.3cm of v34] (v44) {$v^4_{4}$};
\node[draw,        below=.3cm of v44] (v54) {$v^5_{4}$};
\node[draw,        below=.3cm of v54] (v64) {$v^6_{4}$};
%
\node[draw,gray,        right=.6cm of v04] (v05) {$v^0_{5}$};
\node[draw,        below=.3cm of v05] (v15) {$v^1_{5}$};
\node[draw,        below=.3cm of v15] (v25) {$v^2_{5}$};
\node[draw,        below=.3cm of v25] (v35) {$v^3_{5}$};
%
\node[draw,        right=.6cm of v15] (v16) {$v^1_{6}$};
\node[draw,        below=.3cm of v16] (v26) {$v^2_{6}$};
\node[draw,        below=.3cm of v26] (v36) {$v^3_{6}$};
%
\node[draw,        right=.6cm of v16] (v26) {$v^2_{7}$};
\end{tikzpicture}

==> figures/deterministic/do_example_simpl.tex <==
\begin{tikzpicture}
\node[draw] at (0,0)                  (v04) {$v^0_{4}$};
\node[draw,        below=.3cm of v04] (v14) {$v^1_{4}$};
\node[draw,        below=.3cm of v14] (v24) {$v^2_{4}$};
\node[draw,        below=.3cm of v24] (v34) {$v^3_{4}$};
%
\node[draw,        right=.6cm of v04] (v05) {$v^0_{5}$};
\node[draw,        below=.3cm of v05] (v15) {$v^1_{5}$};
%\node[draw,        below=.3cm of v15] (v25) {$v^2_{5}$};
%
\node[draw,        right=.6cm of v15] (v16) {$v^1_{6}$};
%
\draw[->] (v05) -- (v04);
\draw[->] (v05) -- (v14);
\draw[->] (v15) -- (v14);
\draw[->] (v15) -- (v24);
%
\draw[->] (v16) -- (v05);
\draw[->] (v16) -- (v15);
\draw (v16) edge[dashed,->,bend left=20] (v34);
\end{tikzpicture}

==> figures/pariah/pariah_d1.tex <==
\begin{tikzpicture}
\input{figures/pariah/pariah_dag_base}
%
\node[draw,orange, right=.6cm of n52] (n51) {$v^5_{c\phantom{-1}}$};
\draw[orange,dashed] (n02.east) edge[bend left=30] (n51);
\draw[orange,dashed] (n12.east) edge[bend left=30] (n51);
\draw[orange,dashed] (n22.east) edge[bend left=20] (n51);
\draw[orange,dashed] (n42.east) edge[bend left=5] (n51);
\draw[orange,dashed] (n52.east) -- (n51);
\draw[orange,dashed] (n62.east) edge[bend right=5] (n51);
\end{tikzpicture}

==> figures/pariah/pariah_dag_base.tex <==
\node[draw,red] at (0,0)                  (n03) {$v^0_{c-2}$};
\node[draw,        below=.3cm of n03] (n13) {$v^1_{c-2}$};
\node[draw,        below=.3cm of n13] (n23) {$v^2_{c-2}$};
\node[draw,        below=.3cm of n23] (n33) {$v^3_{c-2}$};
\node[draw,        below=.3cm of n33] (n43) {$v^4_{c-2}$};
\node[draw,        below=.3cm of n43] (n53) {$v^5_{c-2}$};
\node[draw,        below=.3cm of n53] (n63) {$v^6_{c-2}$};
%
\node[draw,        right=.6cm of n03](n02) {$v^0_{c-1}$};
\node[draw,        below=.3cm of n02] (n12) {$v^1_{c-1}$};
\node[draw,blue,   below=.3cm of n12] (n22) {$v^2_{c-1}$};
\node[red,draw,    below=.3cm of n22] (n32) {$v^3_{c-1}$};
\node[draw,darkspringgreen,  below=.3cm of n32] (n42) {$v^4_{c-1}$};
\node[draw,        below=.3cm of n42] (n52) {$v^5_{c-1}$};
\node[draw,        below=.3cm of n52] (n62) {$v^6_{c-1}$};
%
\draw[blue] (n03) -- (n22);
\draw[blue] (n13) -- (n22);
\draw[blue] (n23) -- (n22);
\draw[blue] (n33) -- (n22);
\draw[blue] (n43) -- (n22);
%
%\draw[red] (n03) -- (n32);
%\draw[red] (n13) -- (n32);
%\draw[red] (n23) -- (n32);
%\draw[red] (n33) -- (n32);
%\draw[red] (n43) -- (n32);
%
\draw[darkspringgreen] (n23) -- (n42);
\draw[darkspringgreen] (n33) -- (n42);
\draw[darkspringgreen] (n43) -- (n42);
\draw[darkspringgreen] (n53) -- (n42);
\draw[darkspringgreen] (n63) -- (n42);

==> figures/principle/blockchain.tex <==
\begin{tikzpicture}
\node[fill=violet,fill opacity=.25,draw=black,text opacity=1,minimum height=1.75cm, minimum width=.8cm] (b0) at (0,0) {
$
\begin{array}{l}
~
\\
~
\\
~
\\
\end{array}
$
};
%
\node[fill=cyan,fill opacity=.25,draw=black,text opacity=1,minimum height=1.75cm, minimum width=.8cm,right=.5cm of b0] (b1) {
$
\begin{array}{l}
\hline 
x_1
\\
x_2
\\
x_3
\\
\end{array}
$
};
\draw[->] (b1.130) -- (b0.east);
%\draw (b0.290) edge[->,bend right=20,dotted] node[below,yshift=-.1cm,align=center] {$\mathtt{gossip}$ \&\\$\mathtt{consensus}$} (b1.250);
%
\node[fill=red,fill opacity=.25,draw=black,text opacity=1,minimum height=1.75cm, minimum width=.8cm,right=.5cm of b1] (b2) {
$
\begin{array}{l}
\hline 
x_4
\\
x_5
\\
~
\\
\end{array}
$
};
\draw[->] (b2.130) -- (b1.east);
%
\node[above=.05cm of b1] {\footnotesize same order in a Blockchain};
\end{tikzpicture}

==> figures/submit/all_honest.tex <==
\begin{tikzpicture}
\node[circle,draw,inner sep=.5] (n1) at (0,.5) {$A$};
\node[circle,draw,inner sep=.5, below=.5cm of n1] (n2) {$B$};
\node[circle,draw,inner sep=.5, below=.5cm of n2] (n3) {$C$};
%
%\node (lab) at (-.1,1.1) {\footnotesize\shortColGrey{$nodes$}};
%\node[draw,minimum height=2.8cm, minimum width=1cm,dotted] (led) at (-.1,-.2) {};
%
\node[regular polygon,regular polygon sides=5,draw,inner sep=.05cm,outer sep=0cm] (c) at (-.75,.1) {$\chi$};
%
\draw[->] (c.10) -- node[above,pos=.2] {\small$x$} (n1);
\draw[->] (c.10) -- (n2);
\draw[->] (c.10) -- (n3);
%
\node[draw,inner sep=1.5,align=left,right=.5cm of n1] (v1) {$x$\\[-.1cm]$\vphantom{x}.$};
\node[draw,inner sep=1.5,align=left,right=.5cm of n2] (v2) {$\vphantom{x}.$\\[-.1cm]$x$};
\node[draw,inner sep=1.5,align=left,right=.5cm of n3] (v3) {$x$\\[-.1cm]$\vphantom{x}.$};
%
%\node (lab2) at (1.1,1.1) {\footnotesize\shortColGrey{$vertices$}};
%\node[draw,minimum height=2.8cm, minimum width=1cm,dotted] (led2) at (1.1,-.2) {};
%
\draw[->] ($(n1.east) + (0,.1)$) -- ($(v1.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v1) -- (n1);
%\draw[-stealth,gray,dashed] (v1) -- (n2);
%\draw[-stealth,gray,dashed] (v1) -- (n3);
%
\draw[->] ($(n2.east) + (0,.1)$) -- ($(v2.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v2) -- (n1);
%\draw[-stealth,gray,dashed] (v2) -- (n2);
%\draw[-stealth,gray,dashed] (v2) -- (n3);
%
\draw[->] ($(n3.east) + (0,.1)$) -- ($(v3.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v3) -- (n1);
%\draw[-stealth,gray,dashed] (v3) -- (n2);
%\draw[-stealth,gray,dashed] (v3) -- (n3);
%
\end{tikzpicture}

==> figures/submit/one_honest.tex <==
\begin{tikzpicture}
\node[circle,draw,inner sep=.5,fill=cyan] (n1) at (0,.5) {$A$};
\node[circle,draw,inner sep=.5, below=.5cm of n1] (n2) {$B$};
\node[circle,draw,inner sep=.5, below=.5cm of n2] (n3) {$C$};
%
%\node (lab) at (-.1,1.1) {\footnotesize\shortColGrey{$nodes$}};
%\node[draw,minimum height=2.8cm, minimum width=1cm,dotted] (led) at (-.1,-.2) {};
%
\node[regular polygon,regular polygon sides=5,draw,inner sep=.05cm,outer sep=0cm] (c) at (-.75,.1) {$\chi$};
%
\draw[->] (c.10) -- node[above,pos=.2] {\small$x$} (n1);
%
\node[draw,inner sep=1.5,align=left,right=.5cm of n1] (v1) {$x$\\[-.1cm]$\vphantom{x}.$};
\node[draw,inner sep=1.5,align=left,right=.5cm of n2] (v2) {$\vphantom{x}.$\\[-.1cm]$\vphantom{x}.$};
\node[draw,inner sep=1.5,align=left,right=.5cm of n3] (v3) {$\vphantom{x}.$\\[-.1cm]$\vphantom{x}.$};
%
%\node (lab2) at (1.1,1.1) {\footnotesize\shortColGrey{$vertices$}};
%\node[draw,minimum height=2.8cm, minimum width=1cm,dotted] (led2) at (1.1,-.2) {};
%
\draw[->] ($(n1.east) + (0,.1)$) -- ($(v1.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v1) -- (n1);
%\draw[-stealth,gray,dashed] (v1) -- (n2);
%\draw[-stealth,gray,dashed] (v1) -- (n3);
%
\draw[->] ($(n2.east) + (0,.1)$) -- ($(v2.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v2) -- (n1);
%\draw[-stealth,gray,dashed] (v2) -- (n2);
%\draw[-stealth,gray,dashed] (v2) -- (n3);
%
\draw[->] ($(n3.east) + (0,.1)$) -- ($(v3.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v3) -- (n1);
%\draw[-stealth,gray,dashed] (v3) -- (n2);
%\draw[-stealth,gray,dashed] (v3) -- (n3);
%
\end{tikzpicture}

==> figures/submit/one_malicious.tex <==
\begin{tikzpicture}
\node[circle,draw,inner sep=.5,fill=pink] (n1) at (0,.5) {$A$};
\node[circle,draw,inner sep=.5, below=.5cm of n1] (n2) {$B$};
\node[circle,draw,inner sep=.5, below=.5cm of n2] (n3) {$C$};
%
%\node (lab) at (-.1,1.1) {\footnotesize\shortColGrey{$nodes$}};
%\node[draw,minimum height=2.8cm, minimum width=1cm,dotted] (led) at (-.1,-.2) {};
%
\node[regular polygon,regular polygon sides=5,draw,inner sep=.05cm,outer sep=0cm] (c) at (-.75,.1) {$\chi$};
%
\draw[->] (c.10) -- node[above,pos=.2] {\small$x$} (n1);
%
\node[draw,inner sep=1.5,align=left,right=.5cm of n1] (v1) {$\vphantom{x}.$\\[-.1cm]$\vphantom{x}.$};
\node[draw,inner sep=1.5,align=left,right=.5cm of n2] (v2) {$\vphantom{x}.$\\[-.1cm]$\vphantom{x}.$};
\node[draw,inner sep=1.5,align=left,right=.5cm of n3] (v3) {$\vphantom{x}.$\\[-.1cm]$\vphantom{x}.$};
%
%\node (lab2) at (1.1,1.1) {\footnotesize\shortColGrey{$vertices$}};
%\node[draw,minimum height=2.8cm, minimum width=1cm,dotted] (led2) at (1.1,-.2) {};
%
\draw[->] ($(n1.east) + (0,.1)$) -- ($(v1.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v1) -- (n1);
%\draw[-stealth,gray,dashed] (v1) -- (n2);
%\draw[-stealth,gray,dashed] (v1) -- (n3);
%
\draw[->] ($(n2.east) + (0,.1)$) -- ($(v2.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v2) -- (n1);
%\draw[-stealth,gray,dashed] (v2) -- (n2);
%\draw[-stealth,gray,dashed] (v2) -- (n3);
%
\draw[->] ($(n3.east) + (0,.1)$) -- ($(v3.west) + (0,.1)$);
%\draw[-stealth,gray,dashed] (v3) -- (n1);
%\draw[-stealth,gray,dashed] (v3) -- (n2);
%\draw[-stealth,gray,dashed] (v3) -- (n3);
%
\end{tikzpicture}
